From Checking to Inference: Actual Causality Computations as Optimization Problems

Actual causality is increasingly well understood. Recent formal approaches, proposed by Halpern and Pearl, have made this concept mature enough to be amenable to automated reasoning. Actual causality is especially vital for building accountable, explainable systems. Among other reasons, causality reasoning is computationally hard due to the requirements of counterfactuality and the minimality of causes. Previous approaches presented either inefficient or restricted, and domain-specific, solutions to the problem of automating causality reasoning. In this paper, we present a novel approach to formulate different notions of causal reasoning, over binary acyclic models, as optimization problems, based on quantifiable notions within counterfactual computations. We contribute and compare two compact, non-trivial, and sound integer linear programming (ILP) and Maximum Satisfiability (MaxSAT) encodings to check causality. Given a candidate cause, both approaches identify what a minimal cause is. Also, we present an ILP encoding to infer causality without requiring a candidate cause. We show that both notions are efficiently automated. Using models with more than $8000$ variables, checking is computed in a matter of seconds, with MaxSAT outperforming ILP in many cases. In contrast, inference is computed in a matter of minutes.

==> sections/ac3proof.tex <==
Before presenting the proof, we define the term \textit{non-minimal cause}.
\begin{definition} \label{def:non-minmal} \textbf{Non-minimal Cause}\
	is a candidate cause $\vec{X_{(n)}} = \vec{x}_{(n)}$ that satisfies AC2 yet contains at least one element $X_n$ that satisfies one of the following conditions
	\begin{itemize}
		%\item\textbf{NMC1.} Removing $X_n$ from $\vec{X_{(n)}}$ and adding it to $\vec{W}$, results in AC2 holding for the remaining candidate cause $\vec{X}_{(n-1)}$, i.e., $(M,\vec{u})\models \bigl[\vec{X}_{(n-1)}\leftarrow \vec{x}_{(n-1)}',X_n\leftarrow x_n,\vec{W}\leftarrow\vec{w}\bigr]\neg\varphi$
		\item \textbf{NMC1.}  AC2 holds for the smaller cause $\vec{X}_{(n-1)}$ regardless whether $X_n \in \vec{W}$ or not, i.e., $(M,\vec{u})\models \bigl[\vec{X}_{(n-1)}\leftarrow \vec{x}_{(n-1)}',\vec{W}\leftarrow\vec{w}\bigr]\neg\varphi$ and $(M,\vec{u})\models \bigl[\vec{X}_{(n-1)}\leftarrow \vec{x}_{(n-1)}',X_n\leftarrow x_n,\vec{W}\leftarrow\vec{w}\bigr]\neg\varphi$ both hold.
		\item \textbf{NMC2.}  AC2 holds for the smaller cause $\vec{X}_{(n-1)}$ only if $X_n \not\in \vec{W}$, i.e., $(M,\vec{u})\models \bigl[\vec{X}_{(n-1)}\leftarrow \vec{x}_{(n-1)}',\vec{W}\leftarrow\vec{w}\bigr]\neg\varphi$
	\end{itemize}
\end{definition}

Informally, %the first condition covers the case where part of the non-minimal cause should actually be considered in $\vec{W}$. In this case, AC2 does not even hold for the non-minimal cause. 
\textbf{NMC1} deals with irrelevant variables, i.e., those that do not affect the cause relation to the effect. \textbf{NMC2} targets the case of relevant variables that are affected by the cause but not necessary for it to be a cause.
\repeattheorem{ac3}

\begin{proof}
	\begin{proofpart}
		If the cause is a non-minimal cause, then Algorithm \ref{algorithm:fulfillsac3_sat} returns \textit{false}. 	
	\end{proofpart}
	\noindent For the algorithm to return \textit{false}, $G$ must be satisfiable first, and  the cardinality check is passed. So we prove this part by showing that if any of the conditions in Def.\ref{def:non-minmal} hold then $G$ is satisfiable and the check is passed and the algorithm returns \textit{false}.
	\begin{enumerate}
		\item Recall $G := \neg\varphi \wedge \bigwedge_{i=1\ldots\ell} f(U_i=u_i)\wedge\bigwedge_{i=1\ldots m, \not\exists j\bullet X_j=V_i} \left(V_i \leftrightarrow F_{V_i} \lor f(V_i=v_i)\right)	\wedge\bigwedge_{i=1\ldots\ell} (X_i\lor\neg X_i)$. Let us rewrite the formula to abstract the first part as, $G:= G_{base}\wedge\bigwedge_{i=1\ldots n}( X_i\lor\neg X_i)$.  
		\item  Note how  $\vec{X_{(n)}}$ is added to $G$ as $ (X_1 \vee \neg X_1)\wedge(X_2 \vee \neg X_2)\dots (X_n \vee \neg X_n)$. Re-write this big conjunction to have its equivalent disjunctive normal from (DNF) i.e., $ (\neg X_1 \wedge \neg X_2 \dots \wedge \neg X_n) \lor(\neg X_1 \wedge \neg X_2 \dots \wedge X_n)\dots\lor(X_1 \wedge X_2 \dots \wedge X_n)$. Assume wlog
		that all the original values  of $\vec{X_{(n)}}$ (which  lead to $\varphi$ holding true) were \textit{true}, hence to check them in AC2 we present them as negative literals  like $\neg X_i$. Looking at the DNF, we have $2^n$ clauses that list all the possible cases of negating or fixing the elements in $\vec{X}$. Then, we partition $G$ according to the clauses, i.e, $G:=G_1 \lor G_2\dots G_{2^n}$, where $G_1:=G_{base}\wedge (\neg X_1 \wedge \neg X_2 \dots \wedge \neg X_n)$. In the case of the clause where all variables $\vec{X_{(n)}}$ are negated, the corresponding $G$, i.e., $G_1$, is exactly formula $F$ from Algorithm.\ref{algorithm:fulfillsac2_sat}.
		\item Each $G_i$, other than $G_1$, fixes some group of elements to their original evaluation ($X_i$) and negates some, possibly none ($G_{2^n}$), other elements ($\neg X_i$). Clearly, $G_i$ is an $F$ formula (from Algorithm.\ref{algorithm:fulfillsac2_sat}) for all the negated variables, in a clause, as $\vec{X}$ but with x special fixed variables that are added to $\vec{W}$. Hence, a $G_i$ is a check of AC2 for a specific subset of the causes given that the other part (fixed) of the cause is in $\vec{W}$. This is the case of  \textbf{NMC1} in Def.\ref{def:non-minmal}, i.e, AC2 still holds after transferring some elements $\vec{X^*}$ from $\vec{X}$ to $\vec{W}$.  $\vec{X^*}$ is guaranteed to be expressed in one of the $2^n$ clauses, and hence, by a specific $G_k$. According to Theorem.\ref{theorem:F}, such a $G_k$ is satisfiable since AC2 holds. Then, for a non-minimal cause based on \textbf{NMC1}, $G$ is satisfiable since $G_k$ is satisfiable. For this case, we only have to show that it passes the cardinality check in the algorithm. It is clear that  $\forall i \in \vec{X^*} \; v_i' = v_i$ since they will be in $\vec{W}$. This makes the condition in the algorithm evaluates to true and hence, the algorithm returns false. 
		
		
		\item Similarly, for the second case \textbf{NMC2}, i.e., the non-minimal part should not be in $\vec{W}$. AC2 holds for the non-minimal cause, i.e, $F$ and $G_1$ are satisfiable and then $G$ is also satisfiable. Since the non minimal parts in this case are not in $\vec{W}$ or $\vec{X}$, then they follow their equations in the model, and hence $ \exists i \bullet v_i'=[\overrightarrow{V} \mapsto \vec{v}'] F_{X_i}$, which results in false returned by the algorithm. 
	\end{enumerate}
	
	\begin{proofpart}
		If Algorithm\ref{algorithm:fulfillsac3_sat} returns false, then the cause is a non-minimal cause 
	\end{proofpart}
	
	\noindent To prove this part, we show that if $\vec{X}$ is a minimal cause, the algorithm does not return false. The algorithm returns false if $G$ is satisfiable ($\vec{X}$ or a subset of it fulfill AC2), and the cause passes the cardinality check. A minimal cause will have a satisfiable $G$. For the cardinality check, by Lemma.\ref{lemma:negation}, a cause should have all its elements negated. Hence the first conjunct in line \ref{alg:line:fulfillsac3_sat:new_cause} of Algorithm.\ref{algorithm:fulfillsac3_sat} will be \textit{true} for each element. If the second conjunct in the same line ($v_i'\not=[\overrightarrow{V} \mapsto \vec{v}'] F_{X_i}$) evaluates to \textit{false} for any element then, this is not a minimal cause. Hence, for a minimal cause the two conjuncts will evaluate to true for all the elements in $\vec{X}$, and then a false is never returned for such a case. 
\end{proof}



==> sections/approach.tex <==
\section{Approach}\label{sec:approach}
 In  \cite{ibrahim2019}, HP for binary models was encoded in SAT in a way to search for a $\vec{W}$ such that AC2 is fulfilled. We summarize the previous approach, then we present a new SAT approach to handle AC3 without requiring ALL-SAT. Then, we present a novel formulation  of causal checks as an optimization problem that is, first, formulated as an ILP, and then as a maxSAT formula. 
 %Lastly, we wrap-up the section with a comparison of the approaches.


\subsection{SAT 1.0 \protect\footnote{This section is a recap of the approach presented in \cite{ibrahim2019}}}\label{subsec:sat1} 
The first approach to check causality using SAT solving requires constructing and checking \textit{two} SAT formulae, namely $F$ and $G$ to check AC2 and AC3, respectively. The main contribution of \cite{ibrahim2019} lies in how the encoding of AC2  is done in a way that allows for an efficient conclusion of $\vec{W}$.  
Formula $F$ incorporates (1) $\neg\varphi$, (2) a context $\vec{u}$, (3) a setting $\vec{x}'$ for a candidate cause, $\vec{X}$, and (4) a method to infer $\vec{W}$, while still (5) keeping the semantics of the \textit{binary} model $M$.  Since causality analysis is done in hindsight,  the values  $\vec{u}$, and $\vec{v}$ of the variables $\vec{U}$~(size $n$),  and $\vec{V}$ (size $m$) are determined, and we have a candidate cause $\vec{X} \subseteq \vec{V}$ (size $\ell$). The semantics of $M$, given by each function $F_{V_i}$  corresponding to $V_i$ according to Definition~\ref{def:causal_model}, is expressed using the equivalence operator ($\leftrightarrow$)  between the variable and its function, i.e.,  $V_i \leftrightarrow F_{V_i}$. This way  $F$, shown below, is only satisfied for assignments that respect the model semantics.
\begin{small}
\begin{equation*}
F := \neg\varphi \wedge \bigwedge\limits_{i=1\ldots n} f(U_i=u_i) 	\wedge\bigwedge\limits_{i=1\ldots m, \not\exists j\bullet X_j=V_i} \left(V_i \leftrightarrow F_{V_i} \lor f(V_i=v_i)\right)  \wedge\bigwedge\limits_{i=1\ldots\ell} f(X_i=\neg x_i)
\end{equation*} 
\end{small}

 To account for $\vec{W}$  without iterating over the power-set of all variables, we  add a disjunction with the positive or negative literal of each variable $V_i$ to the described equivalence-formula, depending on whether the actual evaluation of $V_i$ was $1$ or $0$, respectively. The actual evaluation of $V_i$ is the value $v_i$ according to its equation $F_{V_i}$ under the context $\vec{u}$. Because $Y_i$ is the variable form, and $y_i$ is the value (true or false), we use the function $f(Y_i = y_i)$ to convert the variable to a positive or a negative literal representation, i.e., $Y$ or $\neg Y$. We present Theorem~\ref{theorem:F} to stress the soundness of $F$ (proof is presented in the supplementary material).
 
\begin{reptheorem}{ac2}\label{theorem:F}
	Formula $F$ constructed with the above encoding is satisfiable iff AC2 holds for a given model $M$, context $\vec{u}$, candidate cause $\vec{X}$, and effect $\varphi$. 
\end{reptheorem}

Checking AC3 is similar to AC2 but with two differences. The first difference is the construction of a new formula $G$, in which each variable of $\vec{X}$ is allowed to take on its original value (actual valuation) \textit{or} its negation (e.g., $A \lor \neg A$). The second difference is the analysis of  $G$'s satisfiability, which requires enumerating \textit{all} the satisfying assignments (All-SAT).  Since $G$ might also be satisfiable for the negated cause $\vec{X} = \vec{x'}$, we cannot conclude that any assignment found, proves that there exists a subset of the cause. Hence,  all of them are needed. Finding an assignment such that at least one conjunct of  $\vec{X} = \vec{x}$ takes on a value that equals the one computed from its  equation, means that it is not a required  part of the cause, and hence the cause is not minimal. The formal construction of $G$ is shown later in Equation~\ref{eq:g} because the coming approaches use it.

%In some situations, this slows down the solver and saturates the memory \cite{toda2016implementing}.

%\begin{reptheorem}{ac3}\label{theo:ac3}
%	Algorithm.\ref{algorithm:fulfillsac3_sat} returns \textit{false} iff $\vec{X}$ is a non-minimal cause.
%\end{reptheorem}

    

\subsection{Optimized AC3 Check with SAT} \label{subsec:sat2}
 Informally, $G$ encodes the set of assignments for $\neg\varphi$ with the removal of the equations for $\vec{X}$. Thus, it can be used to check AC2 (we have all combinations of $\vec{X}$), and to check AC3 by analyzing \textit{all} of them.  This is problematic and decreases the performance if $G$ is satisfiable for a large number of assignments~\cite{toda2016implementing,grumberg2004memory,zhao2009asig}. We present an optimization that eliminates this need by extending $G$ with clauses that encode the notions of \textit{non-minimality} and \textit{non-empty causes}. 
 
  We express \textit{non-minimality} because it is easier to explain than minimality in this context. Non-minimality of a cause means that there exists one variable $X_i= x_i$ in a satisfying assignment of $G$ (which includes $\neg\varphi$, i.e., effect not happening) such that the value of $X_i$  evaluates according to its equation, \textit{or} equals its actual value (i.e., the value for which $\varphi$ evaluates to true) represented as a negative or positive literal. In other words, it is not necessary to negate the value of $X_i$ to have $\neg\varphi$ occurring. We express this notion of non-minimality by the sub-formula  
	$H:= \bigvee ((X_i \leftrightarrow F_{X_i}) \:\lor\: f(X_i=x_i))$.

 The disjunction in $H$ holds if at least one cause variable violates the minimality. On the other hand, a \textit{non-empty} cause means that at least one cause variable $X_j$ is not determined by its equation or takes on its original value, and is negated due to an intervention. We express this notion using  sub-formulas $K$. The first part of $K$ ensures that not all the variables are equal to their original value. The second part ensures that not every variable is allowed to evaluate according to its equation.
 $K:=\neg(\bigwedge f(X_i=x_i)) \land \neg(\bigwedge X_i \leftrightarrow F_{X_i})$.
 




%notion of non-minmal cause and non-empty cause, then added to G to extend it so that it excludes. 
The idea now is to extend $G$ to $G'$ by adding the notions of \textit{non-minimality} ($H$), and \textit{non-empty} cause ($K$), i.e., $G \wedge H \wedge K$. This way, we ensure that $G'$ is only satisfiable if there exists a smaller, and non-empty subset of the cause $\vec{X} = \vec{x}$ that would satisfy AC2. Otherwise, we know that $\vec{X} = \vec{x}$ is minimal. As such, the new clauses make the \textit{unsatisfiability} of $G'$ an indication that AC3 holds. This reduces the analysis effort, and eliminates the need to compute all assignments, but introduces additional clauses when constructing $G'$.



In the following, the  encoding of $G'$ is shown formally.  It starts with the negation of the effect $\varphi$; then it enumerates the context (values of exogenous variables), i.e., $\langle U_1,\ldots,U_n\rangle=\langle u_1,\ldots,u_n\rangle$. Each  variable in $\vec{U}$ is represented as a literal (again using the function $f({Y}={y})$). Then, we use the equivalence operator as explained in Section~\ref{subsec:sat1} to express each  variable ($\langle V_1,\ldots,V_m\rangle=\langle v_1,\ldots,v_m\rangle$) not in the candidate cause. The remainder of the encoding  corresponds to sub-formulas $H$, and $K$ explained above. 
\begin{small}
\begin{equation*}
\begin{aligned}
G' :=  & \neg\varphi \wedge \bigwedge_{i=1\ldots n} f(U_i=u_i)  \wedge\bigwedge_{i=1\ldots m, \not\exists j\bullet (X_j=V_i)} \left(V_i \leftrightarrow F_{V_i} \lor f(V_i=v_i)\right) \wedge H \wedge K
%& \wedge\bigwedge_{i=1\ldots\ell} (X_i\lor\neg X_i) \\
%& \wedge\neg\bigwedge_{i=1\ldots\ell} \left( \neg (X_i \leftrightarrow F_{X_i}) \land \neg (f(X_i=x_i) \right) \\
%& \wedge\neg\bigwedge_{i=1\ldots\ell} (f(X_i=x_i)) 
%  \wedge\neg\bigwedge_{i=1\ldots\ell} (X_i \leftrightarrow F_{X_i})
\end{aligned}
\label{eq:gprime}
\end{equation*} 
\end{small}
%\begin{equation}
%\begin{aligned}
%G* :=  & \neg\varphi \wedge \bigwedge_{i=1\ldots n} f(U_i=u_i) \\
%& \wedge\bigwedge_{i=1\ldots m} \left( \left( \left(V_i \leftrightarrow F_{V_i}\right) \land C_{1i} \right)  \lor \left( \neg \left(V_i \leftrightarrow F_{V_i}\right) \land \neg C_{1i} \right) \right) \\ 
%&\land \left( \left( V_{orig} \land C_{2i} \right)  \lor \left( \neg V_{orig} \land \neg C_{2i} \right) \right) 
%\end{aligned}
%\label{eq:gprime}
%\end{equation} 


% \wedge\neg\bigwedge_{i=1\ldots\ell} \left( \neg (X_i \leftrightarrow F_{X_i}) \land \neg (f(X_i=x_i) \right) \\%


 To check if $\vec{X}$ is a cause of $\varphi$, we need to check $F$ and $G'$ separately, or combine them in one formula ($F \land \neg G'$). The first option allows us to examine each condition (AC2, AC3) in isolation, while the second would report the overall result.  The time for constructing the formulas in the two options is similar, however the CNF conversion and solving time may differ. In our evaluation, we used the first option because it is comparable to the other approaches in being able to distinguish the violation of the two conditions.  Theorem \ref{theorem:g} states the soundness of our encoding (all the proofs of this paper are in the supplementary material). We conclude with the \textit{rock-throwing}  example.
  \begin{reptheorem}{g}\label{theorem:g}
 	Formula $G'$  is satisfiable iff AC3 is violated. 
 \end{reptheorem}
 
 % shows the impact on efficiency as compared to the first approach towards AC3. 
 
 %More importantly, this optimization confirms the result given by Halpern \cite{halpern2015modification} that AC3 can be reduced to an UN-SAT problem. 

%\begin{algorithm}[t]
%	\caption{Check whether AC3 holds using SAT}\label{algorithm:fulfillsac3_sat_optimized}
%	\begin{algorithmic}[1]
%		\Input{causal model $M$, context $\langle U_1,\ldots,U_n\rangle=\langle u_1,\ldots,u_n\rangle$, effect $\varphi$, candidate cause $\langle X_1,\ldots,X_\ell\rangle = \langle x_1,\ldots,x_\ell\rangle$, evaluation $\langle V_1,\ldots,V_m\rangle=\langle v_1,\ldots,v_m\rangle$}	
%		\Function{FulfillsAC3}{$M, \vec{U}=\vec{u}, \varphi, \vec{X} = \vec{x}, \vec{V} = \vec{v}$}
%		\If{$\ell > 1 \land (M, \vec{u}) \models \varphi$}
%		\State\label{alg:line:fulfillsac3_sat_optimized:g}
%		$G' := G  \wedge \bigvee_{i=1\ldots\ell} X_i \leftrightarrow F_{X_i} \:\lor\: f(X_i=x_i)$ \WRP	
%		$ \wedge \neg \bigwedge_{i=1\ldots\ell} f(X_i=x_i) \wedge \neg \bigwedge_{i=1\ldots\ell} X_i \leftrightarrow F_{X_i}$
%		\If{$\textit{SAT}(\textit{CNF}(G'))$}
%		\Return{\textit{false}}\label{alg:line:fulfillsac3_sat_optimized:g_satisfiable}
%		\EndIf
%		\EndIf
%		\State \Return{\textit{true}}
%		\EndFunction
%	\end{algorithmic}
%\end{algorithm}






%\begin{algorithm}[ht]
%	\caption{Check whether AC3 holds using SAT}\label{algorithm:fulfillsac3_sat_optimized}
%	\begin{algorithmic}[1]
%		\Input{causal model $M$, context $\langle U_1,\ldots,U_n\rangle=\langle u_1,\ldots,u_n\rangle$, effect $\varphi$, tentative cause $\langle X_1,\ldots,X_\ell\rangle = \langle x_1,\ldots,x_\ell\rangle$, evaluation $\langle V_1,\ldots,V_m\rangle=\langle v_1,\ldots,v_m\rangle$}	
%	\Function{FulfillsAC3}{$M, \vec{U}=\vec{u}, \varphi, \vec{X} = \vec{x}, \vec{V} = \vec{v}$}
%	\If{$\ell > 1 \land (M, \vec{u}) \models \varphi$}
%	\State\label{alg:line:fulfillsac3_sat_optimized:g}
%		$G := \neg\varphi \wedge \bigwedge_{i=1\ldots n} f(U_i=u_i)$ \WRP 
%		$\wedge\bigwedge_{i=1\ldots m, \not\exists j\bullet (X_j=V_i \land (M, \vec{u}) \models X_j = x_j )} \left(V_i \leftrightarrow F_{V_i} \lor f(V_i=v_i)\right)$ \WRP
%		$\wedge\bigwedge_{i=1\ldots\ell, \not\exists j\bullet ((M, \vec{u}) \not\models X_j = x_j)} (X_i\lor\neg X_i)$ \WRP
%		$\neg \wedge\bigwedge_{i=1\ldots\ell} \left( \neg (X_i \leftrightarrow F_{X_i}) \land \neg (f(X_i=x_i) \right)$ \WRP	
%		$\neg \wedge\bigwedge_{i=1\ldots\ell} (f(X_i=x_i))$ \WRP
%		$\neg \wedge\bigwedge_{i=1\ldots\ell} (X_i \leftrightarrow F_{X_i})$
%		\State\label{alg:line:fulfillsac3_sat_optimized:func}
%		with 	$f({Y}={y}) = \begin{cases}
%		Y,			&y = 1\\
%		\neg Y,	&y=0
%		\end{cases}$		
%		\If{$\textit{SAT}(\textit{CNF}(G))$}
%		\Return{$0$}\label{alg:line:fulfillsac3_sat_optimized:g_satisfiable}
%		\EndIf
%		\EndIf
%		\State \Return{$1$}
%		\EndFunction
%	\end{algorithmic}
%\end{algorithm}

\noindent\textit{\textbf{Example}}:  
We want to check whether $ST = 1 \land BT = 1$ is a cause for $BS = 1$ under $ST_{exo}, BT_{exo} = 1$. Using our encoding, we obtain $G_{ex}'$ (shown below with $H$, $K$ highlighted), which is \textit{satisfiable} for $ST = 0$, $BT = 1$, $SH = 0$, $BH = 0$, $BS = 0$; this is exactly what we wanted to show: $BS = 0$ even if we only set $ST = 0$ while $BT = 1$. Consequently, AC3 does not hold for cause $ST = 1 \land BT = 1$. Note that we can use this result only to check minimality, and not to determine a minimal cause subset because one assignment is not sufficient to conclude a minimal subset.
\begin{small}
\begin{equation*}
\begin{aligned}
&G_{ex}' = \overbrace{\neg BS}^{\neg\varphi} \;\land\; \overbrace{ST_{exo} \land BT_{exo}}^{\vec{u}}
\;\land\; \overbrace{(BS \leftrightarrow SH \lor BH)}^{\text{equation of $BS$}} 
\;\land\; (\overbrace{(SH \leftrightarrow ST)}^{\text{equation of $SH$}} \lor \overbrace{SH}^{\mathclap{\text{orig. $SH$}}}) \;\land \\
&(\underbrace{(BH \leftrightarrow BT \land \neg SH)}_{\text{equation of $BH$}} \lor \underbrace{\neg BH}_{\mathclap{\text{orig. $BH$}}})
\;\land\; \textcolor{blue}{\neg ((\underbrace{\neg(ST \leftrightarrow ST_{exo})}_{\mathclap{\text{negated equ. of $ST$}}} \hspace{2.5mm}\land\hspace{2.5mm} \underbrace{\neg ST}_{\mathclap{\text{negated orig. $ST$}}}) 
	\;\land\; (\underbrace{\neg (BT \leftrightarrow BT_{exo})}_{\mathclap{\text{negated equ. of $BT$}}}} \\& \textcolor{blue}{\hspace{2.5mm}\land\hspace{2.5mm} \underbrace{\neg BT}_{\mathclap{\text{negated orig. $BT$}}}))) \;\land \neg (\underbrace{ST}_{\mathclap{\text{orig. $ST$}}} \hspace{2mm} \land \hspace{2mm} \underbrace{BT}_{\mathclap{\text{orig. $BT$}}}) \;\land\; 
	\neg (\underbrace{(ST \leftrightarrow ST_{exo})}_{\mathclap{\text{equation of $ST$}}} \;\land\;  \underbrace{(BT \leftrightarrow BT_{exo})}_{\mathclap{\text{equation of $BT$}}})}
\end{aligned}
\end{equation*}
\end{small}
\subsection{Actual Causality Query as an Optimization Problem} \label{subsec:ilp}
 The conclusion of the SAT checks aid us in checking whether  $\vec{X}=\vec{x}$ is a \textit{minimal, counterfactual} cause of $\varphi$ or not. This conclusion, however, cannot be used to \textit{infer} a minimal cause in case the candidate cause is not. Thus, we can only answer the \textit{is X a cause of Y?} questions rather than \textit{why did Y happen?}  In this section, we propose a novel strategy to solve a causal query as an optimization problem. Presenting the query as an optimization problem, i.e., an integer \textit{program} or a MaxSat formula, has the advantage of \textit{searching} for a cause rather than checking one answer against the conditions. Using either technique, we check AC2 and AC3 in one round. The result of solving the problem can then be interpreted to conclude the result of  AC2, $\vec{W}$, AC3, and, better, what is a minimal subset of the cause if AC3 is violated. Both techniques are useful in checking minimality, because they solve the program 
 based on an \textit{objective} function.
  

		
%expalin distance
To quantify an \textit{objective} within a causal check,  we introduce an \textit{integer} variable that we call the \textit{distance} variable (formalized in Equation~\ref{eq:distance}). The \textit{distance} is the count of the cause variables ($\vec{X}$) whose value assigned by the (ILP or MaxSat) solver ($x_i'$) is different from their value under the given context (actual evaluation $x_i$ that led to $\varphi$ hold true). Similar to the Hamming distance \cite{hamming1950error}, the distance is a metric to measure the difference between the cause values when $\varphi$ holds true and when it holds false. In other words, we quantify the distance between the actual and the counterfactual world. Equation~\ref{eq:distance} shows the distance as a sum-function of the deltas between variable $X_i$'s actual ($x_i$) and counterfactual value ($x_i'$).  Since an actual cause is non-empty by definition, the \textit{distance} is bounded to have a value greater or equal to $1$.  Further, the distance is less or equal to the size of $\vec{X}$ ($\ell$), i.e., $1 \le distance \le \ell$. Accordingly, we define the \textit{objective function}. Clearly, our objective function is to \textit{minimize} the distance between the actual values of the candidate cause and the computed causes such that the distance is greater than or equal to $1$. As such, we encode a causality check as an optimization problem that aims to \textit{minimize} the number of causes variables while satisfying the constraints for AC2 (counterfactuality and $\vec{W}$). Next, we present the specific ingredients for the ILP formulation, and the MaxSat encoding; then we discuss how to interpret the results to infer a minimal cause from a possibly non-minimal cause. 


\begin{equation}
 distance = \sum_{i=1}^{\ell} d(i) \qquad s.t \qquad d(i) = 
\begin{cases}
1-x_i',& x_i=1\\
x_i',& x_i=0
\end{cases}
\label{eq:distance}
\end{equation}
	

%Specific ILP
\noindent\textbf{ILP.}
To formulate an optimization program using ILP, three elements have to be specified: \textit{the decision variables,  the constraints, and the objective} \cite{brown2007formulating}. Our \textit{decision variables} are, in addition to the \textit{distance} variable,  the set of exogenous and endogenous variables from the model, i.e., $\mathcal{U} \cup \mathcal{V}$. Since we only consider binary variables, those variables are bound to have  values of $0$ or $1$.

Since ILP and SAT solvers can be used as complementary tools,  the translation from SAT to ILP is standard \cite{maknickas2014linear,li2004satisfiability}. Therefore, we reuse formula $G$ (shown in Formula~\ref{eq:g}) to create the ILP \textit{constraints}.  The constraints from $G$ already contain the \textbf{a.)} effect not holding true, \textbf{b.)} exogenous variables set to their values (the context), \textbf{c.)} each endogenous variable either follows the model equation or the actual value, i.e., part of the  set $\vec{W}$, \textbf{d.)} each element in the cause set $\vec{X}=\vec{x}$ is not constrained, i.e., its equation is removed. Transforming these constraints into linear inequalities is straightforward. We do the transformation on the Conjunctive Normal Form (CNF) level. Then, we have clauses that can be reduced to ILP directly. For example, we express $y=x_1 \lor x_2$ as $0 <= 2*y-x_1-x_2 <= 1$~\cite{maknickas2014linear,li2004satisfiability}. In addition to the constraints inherited from $G$,  we add a constraint to calculate the distance according to Equation~\ref{eq:distance}. Lastly, we add an objective function to \textit{minimize} the \textit{distance}.
% by summing the absolute difference between each actual value in $\vec{x}$ and the corresponding value in the ILP solution $\vec{x'}$.
\begin{small}
	\begin{equation}
\begin{aligned}
G :=  \neg\varphi \wedge \bigwedge\limits_{i=1\ldots n} f(U_i=u_i) 	\wedge\bigwedge\limits_{i=1\ldots m, \not\exists j\bullet X_j=V_i} \left(V_i \leftrightarrow F_{V_i} \lor f(V_i=v_i)\right)
\end{aligned}
	\label{eq:g}
	\end{equation} 
\end{small}
\noindent\textbf{MaxSAT.}
The maximum satisfiability problem (MaxSat) is an optimization variant of SAT~\cite{li2009maxsat}. In contrast to SAT solving, which aims to find a satisfying assignment of all the clauses in a propositional formula, MaxSat aims to find an assignment that maximizes the number of satisfied clauses in the formula. As such,  MaxSat allows the potential that some clauses of the formula are unsatisfied. In this paper, we use \textit{partial} MaxSat solving that allows specific clauses to be unsatisfied, referred to as \textit{soft clauses}; contrary to the \textit{hard} clauses that must be satisfied~\cite{li2009maxsat,morgado2013iterative}. Moreover, a soft clause can be assigned a \textit{weight} to represent the cost of not satisfying it. In essence, a weighted partial MaxSat problem is a minimization problem that aims to minimize the cost over all solutions. Unlike ILP, the objective of a MaxSat problem is immutable. Thus, we adapt our formula in a way that achieves the objective function we discussed earlier. 

 %MaxSat is an alternative of 0-1 ILP. 
 %However, the performance of state of the art solvers are remarkably enhancing as can be seen in the MaxSat competition \cite{bibid} especially for the "very boolean" problems. 

%maxsat specific
Similar to the ILP formulation, the MaxSat encoding uses formula $G$ (shown in Formula~\ref{eq:g}) as a base. It embeds the negation of the effect, context, and normal variables, which are all mandatory in any solution. As such, we use the CNF clauses of $G$ as \textit{hard} clauses. On the other hand, we need to append the cause variables ($\vec{X}$) as \textit{soft} clauses. Since the solver would minimize the cost of unsatisfying the ($\vec{X}$) clauses, we represent each cause variable as a literal according to its original value, i.e., $X_{orig}$. Because this is already in CNF, it is easier to assign weights to each clause. We assign $1$ as a cost for unsatisfying the clause $X_{orig}$, i.e., $X$ is negated in the (solved) counterfactual world. Then, the overall cost of unsatisfying parts of the formula is the count of the negated causes, i.e., the size of the minimal cause. Essentially, this concept maps directly to the distance metric that we introduced earlier, which the MaxSat solver will try to minimize by default. Lastly, to ensure that a minimal cause is not empty, we add the non-emptiness clause $K$, from Section~\ref{subsec:sat2}, as a hard clause. Non-emptiness constraint corresponds to defining the lower bound of the distance in ILP.
The MaxSat encoding is shown Formula~\ref{eq:gmax} (soft clauses are underlined).
\begin{small}
\begin{equation}
\begin{aligned}
G_{max} :=  G \wedge \neg(\bigwedge f(X_i=x_i)) \land \neg(\bigwedge X_i \leftrightarrow F_{X_i}) 	 \underline{\wedge\bigwedge\limits_{i=1\ldots\ell} f(X_i= x_i)}
\end{aligned}
\label{eq:gmax}
\end{equation} 
\end{small}

\noindent\textbf{Results.} Once an ILP program or a MaxSat formula is generated, we solve them with a solver such as Gurobi~\cite{gurobi} or Open-WBO~\cite{wbo}. Algorithm~\ref{algorithm:ILP} formalizes the inference of a minimal cause based on the results. The evaluation, in the input, is a list of the variables in $M$ and their values under $\vec{u}$. The rest is self-explanatory.  Assuming $\vec{C}$ is a representation of the optimization problem (a set of linear constraints, or hard/soft clauses), then in Line \ref{alg:line:ilp:assignment}, we solve the program aiming to minimize the \textit{distance}.  We process the results in Lines \ref{alg:line:ilp:x}-\ref{alg:line:ilp:w}. In general, the feasibility of the program or the satisfiability of the formula implies that either $\vec{X}$ or a non-empty subset of it is a minimal cause (fulfills AC2 and  AC3). If \textit{distance}  (cost returned by the MaxSat solver) is equal to the size of $\vec{X}$, then the whole candidate cause is minimal. Otherwise, to infer a minimal cause $\vec{X}_{min}$, we choose the parts that have different values between the actual and the solved values (Line~\ref{alg:line:ilp:x}). At this point, we do not know anything about $\vec{W}$ yet. To determine $\vec{W}$, in Line~\ref{alg:line:ilp:w}, we take all the variables which kept their values the same in the solver solution as in the actual evaluation (potentially including variables from the candidate cause). Obviously, this is not a minimal $\vec{W}$ \cite{ibrahim2019}, which is not a requirement by HP. If the model is \textit{infeasible or unsatisfiable}, then HP for the given candidate cause (and its subsets) does not hold.  Note that an optimization problem can have more than one optimal solution. This implies that multiple minimal causes are found. We collect them all, but we present the first one. To pick one of the causes, we need to employ additional metrics. One possible metric is the responsibility of a cause~\cite{chockler2004responsibility}. 

\begin{algorithm} [t]
	\caption{Interpreting the Optimization Problem's Results}\label{algorithm:ILP}
	\begin{algorithmic}[1]
		\Input causal model $M$, context $\langle U_1,\ldots,U_n\rangle=\langle u_1,\ldots,u_n\rangle$, effect $\varphi$, candidate cause $\langle X_1,\ldots,X_\ell\rangle = \langle x_1,\ldots,x_\ell\rangle$, evaluation $\langle V_1,\ldots,V_m\rangle=\langle v_1,\ldots,v_m\rangle$
		\Function{InferCause}{$M, \vec{U}=\vec{u}, \varphi, \vec{X} = \vec{x},\vec{V}=\vec{v}$}
  		\If{$\langle U_1=u_1\ldots U_n=u_n,V_1=v_1'\ldots V_m=v_m'\rangle =$  $\textit{solve}(\vec{C},\textit{objective})$}\label{alg:line:ilp:assignment}
  		\State $\vec{X}_{min} := \langle X'_1...X'_d\rangle$ s.t. $\forall i\forall j\bullet (i\not= j\Rightarrow$ $X'_i\not= X'_j) \wedge (X'_i=V_j\Leftrightarrow v_j'\not= v_j)$\label{alg:line:ilp:x}
		\State $\vec{W} := \langle W_1...W_s\rangle$ s.t. $\forall i\forall j\bullet (i\not= j\Rightarrow$ $W_i\not= W_j) \wedge (W_i=V_j\Leftrightarrow v_j'=v_j)$\label{alg:line:ilp:w}
		\State \Return{$\vec{X}_{min},\vec{W}$}
		\Else{}
		\Return{\textit{infeasible (unsatisfiable)}}
		\EndIf
		\EndFunction
	\end{algorithmic}
\end{algorithm}
\noindent\textbf{Example:} To illustrate our approach, we show the encodings to answer the query is $ST=1, BT=1$ a cause of $BS=1$? from the rock-throwing example.
\begin{small}
	\begin{equation*}
	\begin{aligned}
	min \enspace d\enspace \textrm{s.t.}& \enspace
	\{BS  =  0,   \enspace ST_{exo} =  1, \enspace BT_{exo} =  1,  \enspace - SH + BS  \geq  0, \enspace - BH + BS \geq  0,  \\&
	\enspace - ST + SH  \geq  0, \enspace BT - BH  \geq  0, \enspace - SH - BH  \geq  -1,
	\enspace ST + BT + d  =  2  \}\\\noindent
	G_{max} = &\neg BS  \;\land\; ST_{exo} \land BT_{exo} \;\land\; (BS \leftrightarrow SH \lor BH)
	\;\land\; ((SH \leftrightarrow ST) \lor SH) \;\land \\ 
	&((BH \leftrightarrow BT \land \neg SH) \lor\neg BH)
	\;\land\;\neg (ST \land BT ) \;\land\; \underline{(ST \land BT)}
	\end{aligned}
	\end{equation*}
\end{small}
Both problems are solved with a  $distance$ (cost) value of  $1$ which indicates that cause $ST,BT$ is not minimal, and there is a minimal cause of size $1$ that can be inferred, namely $ST$. The optimal assignment ($\neg BS, ST_{exo}, BT_{exo}, \neg SH, \neg BH, \\ \neg ST, BT$) showed that the constraints can be guaranteed without having to change the value of $BT$. Thus, it violates AC3. Although this example shows the same result of the SAT-based approach, it shows clearly the enhancement  of the quality of the answer, i.e., finding a specific non-empty, minimal cause rather than only checking the violation of AC3. Theorem \ref{theorem:ilp} states the soundness of our approach (proofs in supplementary material).
\begin{reptheorem}{ilp}\label{theorem:ilp}
 The generated optimization problem (ILP program or $G_{max}$) is feasible iff AC3 holds for $\vec{X}$ or a non-empty subset of $\vec{X}$. 
\end{reptheorem}

\noindent\textbf{Notions of Inference.}

It is clear by now that, in addition to \textit{checking} if a candidate set of variables is an actual cause, we can use our approach to \textit{find} one from within such a set. Based on Algorithm~\ref{algorithm:ILP}, this utilization enables inferring an actual cause, possibly, by constructing a query with a candidate cause that contains all the endogenous leaf variables. Such a candidate cause is probably non-minimal. In cases of multiple solutions (same objective value, i.e., the same cause size), all such causes are collected by our implementation. Still, we currently do not have a mean of comparing these causes during solving (so that the solver picks a cause). Methods to compare causes (such as degree of responsibility~\cite{chockler2004responsibility}) would allow us to get rid of the candidate cause in inference all together; we consider this in the next section.

\section{Causality Inference with ILP} \label{sec:why}
All the approaches, so far, used the candidate cause set $\vec{X}$ somehow. To check AC2 in \autoref{sec:satac2}, we negated the causes in $\vec{X}$; on the other hand, to check AC3 in \autoref{sec:satac3}, we removed the equations corresponding to the cause variables. In this section, we propose another method to \textit{infer} causality without depending on  $\vec{X}$. This approach can be utilized to answer questions of the nature \textit{why $\varphi$?} without hypothesizing anything about the cause. Similar to the ILP approach ($ILP_{is}$), the new method ($ILP_{why}$) uses both propositional formulas and integer linear programming to answer a \textit{why} question. 

% explain the concepts and introduce the formula
In ($ILP_{why}$), we aim to describe the characteristics of an actual cause that have caused an effect $\varphi$. As we have seen so far, this entails translating the conditions of HP (according to \autoref{def:ac}). However, since the conditions depend on the existence of a candidate cause $\vec{X}$, ($ILP_{why}$) formulates the problem differently. We will leverage the metric of \textit{responsibility} which was introduced earlier in \autoref{sec:responsibility}. Expressing responsibility as a numeric value that quantifies the degree that a cause contributes to an effect is the base of this work. Because we can have multiple causes in which the three HP conditions hold given a  model and a context, we can compare such causes according to their degree of responsibility. In other words, we instruct the solver to \textit{find} a cause with the \textit{maximum} degree of responsibility. We come back to this goal after we construct a formula $G^*$ that is the base of $ILP_{why}$. 


% the new concept is to use a formula again; then add auxilairy vars and ojectives; do i use the distance?
Analogous to all the previous formulas, we start our construction with the negated effect formula ($\neg\varphi$), and inclusion of the context $f(U_i=u_i)$. To continue with a \textit{why} query, we have two classes of endogenous variables: \textbf{1.} variables that belong to the effect formula, and \textbf{2.} all the other variables. Because the effect variables are not supposed to be part of the cause (check if this per definition), we can represent the first group with the \textit{equivalence} relation, i.e., $V_i \leftrightarrow  F_{V_i}$. The interesting part is the representation of the other variables. Since we are looking for the cause set, we need to allow each variable to be in one of the three categories: \textbf{a.} a cause variable, \textbf{b.} a contingency-set variable, \textbf{c.} a normal variable. In a counter-factual computation, a cause variable does not follow its equation, \textit{and} differs from its original value. A contingency-set variable, on the other hand,  does not follow its equation while keeping its original value. A normal variable does follow its equation, regardless of whether being equal to the original value or not. To generalize, each variable $V_i$ is represented as a disjunction between the equivalence holding and not holding, \textit{and} a disjunction between its original value and its negation. This is shown in \autoref{eq:vars}.    
\begin{equation}
	\begin{aligned}
		& \left(  \left(V \leftrightarrow F_{V}\right)   \lor  \neg \left(V\leftrightarrow F_{V}\right)  \right) 
		\wedge \left(   V_{orig} \lor \neg V_{orig} \right) 
	\end{aligned}
	\label{eq:vars}
\end{equation} 
Clearly, each clause in the previous equation is a tautology. However, this generalization enables the classification of the variables in the three categories; more importantly, we incentivize the solver to classify those variables according to criteria. 


To possess  the ability to guide the solver's behavior, we need a method to control how each variable is solved. Thus, we add auxiliary boolean variables to each of the clauses. These variables are crucial for two purposes. First, we use them as \textit{indicators} to conclude which clauses hold. Since the first disjunction is not mutually exclusive with the second, i.e., a variable can follow its equation, yet have its original value, we need \textit{two} auxiliary control variables. Secondly, similar to the concept of \textit{distance} from \autoref{subsec:ilp}, we use the auxiliary variables to describe the criteria of the solution.  

We add two control variables $C_1$, and $C_2$. The variables are appended to the four clauses presented before. Each endogenous variable is then presented as:
\begin{equation}
	\begin{aligned}
		&  \left( \left( \left(V \leftrightarrow F_{V}\right) \land C_{1} \right)  \lor \left( \neg \left(V \leftrightarrow F_{V}\right) \land \neg C_{1} \right) \right) 
		&\land \left( \left( V_{orig} \land C_{2} \right)  \lor \left( \neg V_{orig} \land \neg C_{2} \right) \right) 
	\end{aligned}
	\label{eq:vars2}
\end{equation} 
As such, the class of each endogenous variable can be determined based on its control variables values. For example, a variable with a $C_1$ equals $1$ is a normal variable that follows its equation. Otherwise, it is a cause variable if its $C_2$ is $0$. \autoref{tab:controlVars} shows all the cases of the control variables and their corresponding classification. Finally, the  overall formula $G^*$ is shown in \autoref{eq:gstar}. 


\begin{table}[!ht]
	\centering
	%\resizebox{0.2\textwidth}{!}{%
	\begin{tabular}{|c|c|c|}
		\hline
		C1 & C2 & Variable \\ \hline
		0 & 0 & Cause \\ \hline
		0 & 1 & Contingency Set ($\vec{W}$) \\ \hline
		1 & 0 & \multirow{2}{*}{Normal} \\ \cline{1-2}
		1 & 1 &  \\ \hline
	\end{tabular}%
	%}
	\caption{The Truth Table of the Control Variables}
	\label{tab:controlVars}
\end{table}



\begin{equation}
	\begin{aligned}
		G^* :=  & \neg\varphi \wedge \bigwedge_{i=1\ldots n} f(U_i=u_i) \\
		& \wedge\bigwedge_{i=1\ldots m} \left( \left( \left(V_i \leftrightarrow F_{V_i}\right) \land C_{1i} \right)  \lor \left( \neg \left(V_i \leftrightarrow F_{V_i}\right) \land \neg C_{1i} \right) \right) \\ 
		&\land \left( \left( V_{orig} \land C_{2i} \right)  \lor \left( \neg V_{orig} \land \neg C_{2i} \right) \right) 
	\end{aligned}
	\label{eq:gstar}
\end{equation} 

%objectives
% main concept
%Objective1:  Maximize responsibility, i.e., minimize X+W
%Objective 2: Minimize the number of cause variables X  
%For variables that follow their equations C1 is true (regardless of C2) Variables in W, C1 is false and C2 is true,  Variables in X, C1 and C2 are false 
%Max multi-objectives
%OBJ0: Priority=2 Weight=1 AbsTol=0 RelTol=0
%C1_sum
%OBJ1: Priority=1 Weight=1 AbsTol=0 RelTol=0
%C1_com_sum - C3_sum

So far, we have shown the construction of the formula and its parts that correspond to the constraints of the optimization problem. The important step is to define the \textit{objective} of this formulation. As mentioned, we want to find an assignment to the constraints shown in $G^*$ that corresponds to a cause with a maximum degree of responsibility. Let us recall the degree of responsibility as given in \autoref{def:respo} is $\dfrac{1}{|X|+|W|}$. Thus, \textit{maximizing} the responsibility entails \textit{minimizing} the sizes of both the cause and the contingency sets, i.e., $|X|+|W|$. Since the sizes of the three (cause, contingency, and normal) sets of variables 
form the overall model size (excluding the effect variables), then minimizing $|X|+|W|$ is equivalent to maximizing the number of normal variables.  The sum of values of $C_1$ variables  represents the number of normal variables; thus, the objective is to \textit{maximize} the sum of $C1$ variables.  

% introduce the objectives and the  hierarchical    
% give an algorithm; how to read the results; the problem
The problem of our formulation so far is that it tries to minimize $\vec{X}$, and $\vec{W}$ as a whole. Rather, we would aspire to distinguish them. Assume, for example, we have two witnesses \footnote{Recall a witness is a tuple of $(\vec{W}, \vec{w}, \vec{x'})$} one with a cause set of size $2$ and a $\vec{W}$ of size $3$, and the second witness with a cause set of size $3$ and a $\vec{W}$ of size $2$. The two causes will be considered as an optimal solution to the problem; however, ideally, we would like to pick the first witness since it has  fewer causes. Thus, we alter our formulation to add a new objective. ILP works with multiple objectives in two modes, hierarchical or blinded~\cite{ilp}. We use hierarchical Objectives in which the solver optimizes the problem given the first objective and then use the second objective to find the optimal solution among the solutions with the same first objective value. The second objective in our formulation is to \textit{minimize} the number of causes, i.e., the number of variables with $C_1$ and $C_2$ equal to $0$. The second objective required a third control variable, i.e., $C_3$ that captures the case when the first two control variables are $0$. In other words, $C_3= \neg C_1 \wedge \neg C_2$. 




%With multiple objectives, we need to optimize the optimal solution of first objective. The exact thing to be optimized is the 
%number of causes. We cannot directly infer that from c1 or c2 alone, since we need to count the number of ~c2 given ~c1. The 
%linear representation of this is on the expense of adding another variable c3 for each variable. This variable is equal to 
%~c1 and ~c2. This will be add 2 constraints per variable. The sum of c3 will be the size of X, variables for which c3 is 1 will be a cause.

\subsubsection{$Why_{ILP}$ Algorithm}
We have discussed the building blocks of the formulation to infer causality based on responsibility. In this section, we wrap-up the approach with the Algrothim~\autoref{algorithm:why}. It follows a construction similar to Algorithm~\autoref{algorithm:ILP}; however, without the dependency on a candidate cause set in the input.  

\begin{algorithm} [t]
	\caption{Causality Inference using $Why_{ILP}$}\label{algorithm:why}
	\begin{algorithmic}[1]
		\Input causal model $M$, context $\langle U_1,\ldots,U_n\rangle=\langle u_1,\ldots,u_n\rangle$, effect $\varphi$, evaluation $\langle V_1,\ldots,V_m\rangle=\langle v_1,\ldots,v_m\rangle$
		\Function{FindCause}{$M, \vec{U}=\vec{u}, \varphi, \vec{V}=\vec{v}$}
		\State{ \label{alg:line:why:g}
			$G^* :=   \neg\varphi \wedge \bigwedge_{i=1\ldots n} f(U_i=u_i) \wedge \bigwedge_{i=1\ldots n, V_i \in \varphi} (V_i \leftrightarrow F_{V_i})$ \WRP $\wedge\bigwedge_{i=1\ldots m, V_i \not\in \varphi} \left( \left( \left(V_i \leftrightarrow F_{V_i}\right) \land C_{1i} \right)  \lor \left( \neg \left(V_i \leftrightarrow F_{V_i}\right) \land \neg C_{1i} \right) \right)$ \WRP  
			$\land \left( \left( f(V_i= v_i)  \land C_{2i} \right)  \lor \left( f(V_i= \neg v_i)  \land \neg C_{2i} \right) \right)$}	
		\State{ \label{alg:line:why:constraints}
			$\langle C_1=c_1\ldots C_n=c_n \rangle =$  $\textit{convertToILP}(\textit{CNF}(G^*))$	}
		\State{ \label{alg:line:why:objective}
			$\textit{objective}_1 = Maximize\;  \sum_{i=1}^{m} C_{1i}\;  s.t.\;  \textit{objective}_1 \leq |\vec{V}|$} 
		\State{ \label{alg:line:why:objective2}
			$\textit{objective}_2 = Minimize\; \sum_{i=1}^{m} C_{3i}\;  s.t.\;   |\vec{V}|  => \textit{objective}_2 >=1$}
		\If{$\langle V_1=v_1'\ldots V_m=v_m', C_{11}= c_{11}'\ldots  C_{1m}= c_{1m}', C_{21}= c_{21}'\ldots  C_{2m}= c_{2m}', $ \WRP $C_{31}= c_{31}'\ldots  C_{3m}= c_{3m}' \rangle = \textit{solve}(\vec{C},\textit{objective}_1, \textit{objective}_2)$}\label{alg:line:why:assignment}
		\State $\vec{X'} := \langle X'_1...X'_{obj_{2}}\rangle$ s.t. $\forall i\forall j\bullet (i\not= j\Rightarrow$ $X'_i\not= X'_j) \wedge (X'_i=V_j\Leftrightarrow c_{3j}'= 1)$\label{alg:line:why:x}
		\State $\vec{W} := \langle W_1...W_s\rangle$ s.t. $\forall i\forall j\bullet (i\not= j\Rightarrow$ $W_i\not= W_j) \wedge (W_i=V_j\Leftrightarrow ( c_{1j}'= 0 \wedge  c_{2j}'= 1  ))$\label{alg:line:why:w}
		\State \Return{$\vec{X'},\vec{W}$}
		\Else{}
		\Return{\textit{infeasible}}
		\EndIf
		\EndFunction
	\end{algorithmic}
\end{algorithm}

The algorithm starts with constructing the formula $G^*$ in \autoref{alg:line:why:g}. The choice to depend on a propositional formula to express the constraints of the equation seemed natural, given our previous approaches. Because of the complexity of $G^*$ in terms of the number of clauses that represent each variable, this dependency is a potential bottle-neck (more on that in the evaluation). To start formulating the query as an integer program, we turn the conjunctive normal form of $G^*$ into a set of linear constraints in \autoref{alg:line:why:constraints}. We then complete constructing the program, in \autoref{alg:line:why:objective}-\autoref{alg:line:why:objective2}, by adding the objectives. The first objective of the program, i.e., $\textit{objective}_1$ concerns maximizing the degree of responsibility which, as discussed earlier, corresponds to maximize the sum of all the control variables $C_1$. The second objective, $\textit{objective}_2$, handles minimizing the size of the cause set, which is equivalent to the sum of the control variables $C_3$. 

Lastly, we process the results after solving the program in \autoref{alg:line:why:assignment}-\autoref{alg:line:why:w}. To reflect the assignments returned by the solver to answer a \textit{why} query, we check the control variables. Generally, the feasibility of the program means that there is a cause of size at least 1 (exact size is $\textit{objective}_2$), which makes phi not hold, under the given context.  The set of causes variables  can be inferred by checking $C_3$ corresponding to each endogenous variable, and those variables that have a $C_3$ that equals $1$ are causes. The contingency set, i.e., $\vec{W}$, can be inferred by checking the first two control objects $C_1, C_2$. When $C_1$ equals $0$, and $C_2$ equals $1$, the corresponding variable should be added to the contingency set.



%To process the results:
%//		1- c1sum is the number of normal variables (evaluate according to their equations), for the exact variables check the C1_Vi=1
%//		2- c3sum is the size of the cause vector, the exact variables can be deducted by collecting C3_Vx=1 variables  
%//		3- W size can be calculated using the above(complement-c3sum) , for the exact variables check C1_Vi and C2_Vi should be 01
%// OPTIMAL 2 Model was solved to optimality INFEASIBLE 3 Model was proven to be
%// infeasible.


%TODO: for a theorem
\subsubsection{Example}
To illustrate the approach, using the rock-throwing example,  \autoref{fig:ilpwhy} shows the generated program for a why query. The query is  \textit{why did the bottle shatter $BS=1$?} 
\begin{small}
	\begin{equation}
		\begin{array}{lll}
			&\displaystyle \max_{C1SUM} 	&\displaystyle \min_{C3SUM} \\
			&\textrm{s.t.} 					 &BS  =  0 \\
			&ST_{exo}  =  1 &BT_{exo}  =  1 \\
			&-BS + SH + BH  \geq  0 	&BS - SH  \geq  0  \\  
			&BS - BH  \geq  0 	&C1_{SH} - AT - SH  \geq  -1 \\  
			&C1_{SH} + SH + AT  \geq  1 &-SH + AT - C1_{SH}  \geq -1 \\  
			&SH - AT - C1_{SH}  \geq -1 &C2_{SH} - SH  \geq  0  \\  
			&SH - C2_{SH} \geq  0 &C1_{BH} - BT + SH - BH  \geq  -1\\  
			&C1_{BH} + BH + BT  \geq  1 &C1_{BH} + BH - SH  \geq  0 \\  
			& -BH + BT - C1_{BH}  \geq  -1 	& -BH - SH - C1_{BH}  \geq  -2 \\ 
			& BH - BT + SH - C1_{BH}  \geq  -1 	& C2_{BH} + BH  \geq 0 \\  
			& -BH - C2_{BH} \geq  -1 & C1_{ST} - ST_{exo} - AT  \geq  -1 \\  
			& C1_{ST} + AT + ST_{exo}  \geq 1 & -AT + ST_{exo} - C1_{ST}  \geq  -1 \\  
			& AT - ST_{exo} - C1_{ST}  \geq  -1 & C2_{ST} - AT  \geq 0 \\  
			& AT - C2_{ST}  \geq  0 	& C1_{BT} - BT_{exo} - BT  \geq  -1 \\  
			& C1_BT + BT + BT_{exo}  \geq  1 & -BT + BT_{exo} - C1_{BT}  \geq  -1 \\  
			& BT - BT_{exo} - C1_{BT}  \geq  -1 & C2_{BT} - BT  \geq  0 \\  
			& BT -C2_{BT}  \geq  0 	& - C^1_{BT} - C2_{BT} - 2 C3_{BT} < =  -1 \\
			& - C1_{BT} - C2_{BT} - 2 C3_{BT}   \geq  -2 & - C1_{BH} - C2_{BH} - 2 C3_{BH} < =  -1 \\
			& - C1_{BH} - C2_{BH} - 2 C3_{BH}   \geq  -2 & - C1_{SH} - C2_{SH} - 2 C3_{SH} < =  -1 \\ 
			& - C1_{SH} - C2_{SH} - 2 C3_{SH}   \geq -2 & - C1_{ST} - C2_{ST} - 2 C3_{ST} < =  -1 \\
			& - C1_{ST} - C2_{ST} - 2 C3_{ST}   \geq  -2 & C1_{BT} + C1_{BH} + C1_{SH} + C1_{ST} - C1_{sum}  =  0 \\
			&C1_{sum} + C1_com_{sum}  = 4 & C3_{BT} + C3_{BH} + C3_{SH} + C3_{ST} - C3_{sum} =  0	 \\
			%				& V_i  \in [0,1] &\forall& V_i \in V,& distance  \in  [1,2]  &  \\
		\end{array}
		\label{eq:ilpwhy}
	\end{equation}
\end{small}

The solution of the program is shown in \autoref{eq:whysol}. From the set of variables not included in the effect formula, we have \textit{two} normal variables based on the sum of $C1$ variables ($C1_{sum} = 2$). On the other hand, we have two variables that are are part of either $\vec{X}$, or $\vec{W}$, shown by the value of the complement of $C1_{sum}$. More importantly, we see that the cause set size is $1$ according to the sum of $C3$ variables ($C3_{sum}$). To infer the specific cause and contingency set variables, we look at the specific control variables. Based on the truth table of \autoref{tab:controlVars}, $SH=1$ is the actual cause of $BS=1$, given that $BH=0$. This is the result of having $C3_{SH}= 1$ which corresponds to $C1_{SH} = 0 \wedge C2_{SH} =0 $ as opposed to $C1_{BH} = 0 \wedge C2_{BH} = 1$. 

\begin{equation*}
	\begin{array}{lllll}
		C1_{sum} = 2 &	C1_{com_sum} = 2 &	C3_{sum}   = 1&&\\ 
		ST_{exo}=1 & 	BT_{exo} = 1 & BS=0 &&\\
		SH  =  0 & 	C1_{SH}  =  0& C2_{SH}   =  0& C3_{SH}   =  1&  \\
		BH  =  0&	C1_{BH}  =  0& C2_{BH}  =  1& C3_{BH}  =  0&  \\
		ST  =  1& 	C1_{ST}  =  1& C2_{ST}  =  1& C3_{ST}  =  0&  \\
		BT  =  1&	C1_{BT}  =  1& C2_{BT}  =  1& C3_{BT}  =  0&   \\		
	\end{array}
	\label{eq:whysol}
\end{equation*}

%  C1_sum 2  %C1_com_sum     2 %C3_sum  1 %ST_exo   1 %BT_exo   1 %AT  1 %BT 1%C2_BH 1 %C1_AT  1 %C2_AT  1 %C1_BT  1%C2_BT    1%C3_SH   1
The results returned by the approach are correct. $SH$ is an actual cause of $BS$, according to HP. Under the given context, the inferred cause has a maximum degree of responsibility ($\dfrac{1}{2}$). All the instances of this example referred to $ST$ as the actual cause; however, since the equation of $SH$ is an identity function ($SH=ST$), this does not compromise our result. Arguably, the depth of the cause, the (geodesic) distance between the nodes in the graph, can be taken into consideration. In this thesis, we do not consider this issue.  






==> sections/xai.tex <==
Introduction in General

The rapid deployment of digital systems into all aspects of our daily life has incited the need for embedding human’s social constructs into the digital world.  Many of those social concepts, like explanation, accountability, and ethics, rely on some notion of causal reasoning. In systems based on artificial intelligence, the public is interested in \emph{explaining} decisions, recommendations, or predictions that result from such systems. In safety or security critical systems, people are keen on holding miss-behaving parties responsible for any violation.  Similarly, in future autonomous systems, manufacturers are trying to design their systems to behave ethically. For all such goals, the need to reason about the causality is universal regardless of whether it was a \emph{cause} of a decision made by the system, a \emph{cause} of a safety incident, or the ethical judgment of a  \emph{consequence} resulting from an autonomous car action.  


Actual causation theories typically discuss three main ingredients: a model,  context, and a reasoning mechanism. Causal modeling refers to abstracting and representing a  general knowledge of cause and effect relations, while context setting refers to a specific assignment of the model, and finally, reasoning refers to the process of inferring actual causation using the models and the contexts. We argue that the first two ingredients interweave the social and technical boundaries of systems since they potentially include making explicit human knowledge, or monitor human-related activities. However, when formalized -like in the case of Halpern and Pearl definition of actual causality-,  the reasoning part can be seen as a technical concept solely. In this paper, we focus on how to build an efficient, and scalable causality reasoning mechanism that can, then, be utilized in different domains and for different purposes. 
%- efficient computation why ? where are the big models


\section{Explainable AI models}

- growth of the field, the motivation behind the need for it 

- insights from social sciences suggest the need for human-like ways of explanation [Miller, Mittelstadt]. accounts of explanation are given, HP is seen as a potentail.

- There are many apparent challenges before we reach there, like: precise modeling, what are the scopes of the explanations, complexity, bridging the gap of the contrastive queries and causal queries, giving efficent ways that should also scale to size of ML models


- Related work on xai and interpretability, scientific models [Mittelstadt]  are not enough, people consider contrastive .... some work [Narendra] gives a way to create a causal model from CNN

- work should be on making explicit what is the query like especially the phi... levels or scopes of queries, 





\paragraph{transformation} To illustrate the approach, we start with a simple example to classify different types of arthropods \cite[miller]; the example was introduced by Miller \cite{miller}, and later on by Mittelstadt \cite{mittelstadt}. The example shows the features and the parameters learned by machine learning algorithm to classify arthropods. Note that some of the features are binary features like the fact that the arthropod has a stinger or not. Other features are integer-based like the number of legs. Since we only support binary models, we use binary representation of the integer values. Although there maybe other elegant way to handle decimal features, we think that a binary model captures everything we want to explain, e.g., in the example the fact that an arthropod has eight legs makes the algorithm classify it as a spider, the number \textit{eight} is not needed in an arithmetic way . Furthermore, we think that the growth of the model, due to the auxiliary variables that we add to binarize the decimal values, is acceptable in comparison to the computational complexity of causal reasoning of non-binary models \cite{complexity}. 
   
In this section, we discuss the conceptual and technical ingredients of causality checking in the domain of machine-learning. Conceptually, supervised machine-learning  approaches generate models to decide on new data instances. Explanation for such approaches would seek to understand, for example,  why classification $P$ was returned. From causality perspective, this is an actual cause query \cite{halpern2016actual}. It tries to look for \emph{causes} of an already observed \emph{effect}. For such queries, three ingredients are needed: a representation of the classifier causal behavior, i.e., a causal model, the exact information about the classified point, i.e., the context, and lastly, the reasoning machinery to use the first two ingredients to answer causal queries. In this paper, we show one possible transformation to causal models, and a complete efficient reasoning algorithm to explain artificial intelligence approaches.   

\paragraph{causal model} Depending on the used machine-learning algorithm, different representations of the learned models are possible. In this paper, we use the one presented in the example, i.e., a tabular set of features and the values that correspond to one class. Each class, and feature is presented as an endogenous variable. To accommodate for their values, a feature variable may be presented by a set of variables, corresponding to its bits. For example, the number of wings (N.W) feature can have the values $0$, $2$, or $4$, hence it will represented with \textit{two} variables $N.W_1, N.W_0$. The different binary values of the two bits will correspond to an index of the real values, i.e., $00$ means $0$, $01$ means $5$, and $10$ means $4$. Please note that we are not transforming the decimal values appearing in the table to their binary representation, but rather we are assigning them a binary value that consists of some number of bits. The number of bits, and then the number of variables, depend on the number of distinct values that we need to present. In the example about $N.W$, we have three values and hence we use two bits. This way we use less number of variables. There are more rigorous ways to express non-propositional relations in boolean logic like the Ackermann reduction \cite{ackermann}, this approach can be seen as one-case of this reduction. For the exogenous variables, we express each feature (or set of feature bit variables) with its own exogenous variables. 

\begin{figure}
	\includegraphics[scale=0.9]{./figs/table.png}
	\caption{A screen shot of the table}
	\label{fig:mltable}
\end{figure}

In addition to the variables, we create the propositional equations from the table. For instance, a spider is an arthropod that has eight legs, \textit{and} not stinger, \textit{and} 8 eyes, and no compound eyes, and zero wings. Then, each class variable is a conjunction of the features value, i.e., $spider = (no.wings=0) \wedge (!stinger)... $. Note that $(no.wings=0)$ is presented as explained above. As such, we create a simple causal structure of the factors leading to classifying an arthropod. This paper focuses on how to compute causality given such structures. That said, we think that there are still a couple of questions that are worth tackling in future work. The main question is how do we take into consideration the variance of the importance of the features, i.e., the weights of these features. Potentially, a candidate to represent the variance is considering them in light of preemption cases \cite{halpern2016actual}.    

\begin{figure}
	\includegraphics[scale=0.9]{./figs/binarrepop1.png}
	\caption{The causal graph of the example}
	\label{fig:mlcm}
\end{figure}

With the informal discussion above, we now present the causal model of the example in Figure~ \ref{fig:mlcm}. Given this model, we can now provide explanations about specific classifications. For an AI system, the specific case (an image of an arthropod) is seen as a vector of features. This is precisely the \textit{context} of a causal query. Formally, the context is an assignment of the exogenous variables, which we can easily see that it maps to the values of the features we consider. For example, \textit{image J} contains no wings, and 8 legs. What remains is phrasing the causal query. Miller \cite{miller2018} argues that human perception of explanation often refers to a contrastive question, i.e., why $P$ rather than $Q$. We think such a question can be formulated using HP by focusing on what is the effect $\varphi$. In HP, an effect can be any boolean combination of variables; the most basic contrastive question can then be seen as $(P \wedge \neg Q)$. The result of the causal question -according to HP it is a witness world formally $(\vec{X},\vec{x'}, \vec{W})$- can then be considered a contrastive explanation.

 Let us consider an example question: \textit{ why is image J labeled as a Spider instead of a Beetle?} Assume the feature vector of the image is (...). Note that if we want to consider the image recognition as part of the explainable system, we then have to also create a causal model for it or expand the model in Figure~\ref{fig:mlcm} to describe its behavior. 




 
